A Deep Reinforcement Learning Approach to First-Order Logic Theorem Proving

Automated theorem provers have traditionally relied on manually tuned heuristics to guide how they perform proof search. Deep reinforcement learning has been proposed as a way to obviate the need for such heuristics, however, its deployment in automated theorem proving remains a challenge. In this paper we introduce TRAIL, a system that applies deep reinforcement learning to saturation-based theorem proving. TRAIL leverages (a) a novel neural representation of the state of a theorem prover and (b) a novel characterization of the inference selection process in terms of an attention-based action policy. We show through systematic analysis that these mechanisms allow TRAIL to significantly outperform previous reinforcement-learning-based theorem provers on two benchmark datasets for first-order logic automated theorem proving (proving around 15% more theorems).

==> app-hyperparam.tex <==
\section{Appendix - Hyper-Parameter Tuning}
We used gradient-boosted-tree  search  from
scikit-optimize~\footnote{https://scikit-optimize.github.io/} to  find  effective  hyper-parameters using 10\% of of Mizar40 dataset. We present here the list of hyper-parameters as well as their value range provided as input to the hyper-parameter tuning algorithm. We also  present the list of all hyper-parameter values used in our experiments.

\begin{table*}
  \caption{Hyper-Parameter Ranges and Values Used } 
  \label{tab:hyperparams_tunable}
  \centering
  \resizebox{0.9\columnwidth}{!}{%
    \begin{tabular}{|l|l|l|}
        \hline
        Name & Value Range & Value Used\\  \hline
        $k$ (number of layers) & Integer([0, 30]) & 2 \\
        Units per layer & Integer([25, 200]) & 161 \\
        Activation function & \{ReLU\} & ReLU \\ 
        $2d$ (sparse vector size) &  Integer([10, 1000]) &  645 \\
        Dropout probability & Real([0, 0.6]) &  0.57 \\
        $\lambda$ (entropy reg.) & \{0.0, 0.002, 0.004, 0.008, 0.016, 0.032, 0.064, 0.128\} & 0.004 \\
        $\tau$ (temperature) & Real([1, 5])  & 1.13\\
        $\tau_0$ (temperature threshold) & Integer([10, 50]) & 11 \\
        Temperature decay factor & Real([.95, 1]) & 0.9998\\
        $\rho$ (expert reliance decay) & Real([0.1, 0.99]) & 0.75 \\
        Reward Normalization & \{No Norm, Norm. w.r.t. Beagle #steps, Relative Norm. w.r.t. best attempt\} & No Norm \\
        Treat constants as functions in vectorization & \{TRUE, FALSE\} & TRUE\\ 
        Optimizer & \{Adam(betas = (0.9, 0.999), weight decay = 0, eps = 10^{-8})\} & Adam \\
        Learning rate & \{0.001\} & 0.001  \\
        Batch size & \{32\} & 32 \\
        Number of epochs & \{15\} & 15 \\
        $w$ (keep examples from the last $w$ iterations) & \{20\} & 20 \\
        \hline
    \end{tabular}
    }
\end{table*}

Table~\ref{tab:hyperparams_tunable} below shows the list of   hyper-parameters. For each hyper-parameter, we show  its value range and the value used in our experiments. 




==> sections/discussion.tex <==
\section{Discussion and Future Work}

\textbf{Action Space} In typical RL setups such as games, the action space is fixed, finite and does not change in each step. However, fixing the action space in theorem proving is very challenging. In our case, we opted to have actions representing the candidate clauses to be selected at each step which made that space grows and shrink as the episode progresses. Having actions as inference rules, for example, will make the action space finite and fixed. However, this will require an extra module to select which clauses to apply the rule on, and, although at a given reasoning step the number of candidate clauses is finite, the number of candidate clauses that can be produced during a proof attempt is not bounded as new clauses are constantly produced during the reasoning process. As part of our future work, we are exploring a number of techniques that can fix or limit the action space during theorem proving. 

\textbf{Reward Function} We experimented with two types of reward functions. The first one is based on the number of steps used to find a proof while the second one is based on the amount of time spent. The advantage of time-based reward is that it implicitly encapsulate all the other costs associated with picking an action such the complexity of executing  action and how much much clauses it generate. We found empirically that both types of rewards reach the same performance eventually with time-based reward converging much faster. 


\ibrahim{add future work: behavioral cloning, other RL algorithms, extension to HOL} 

